DeFi: data-driven characterisation of Uniswap v3 ecosystem & an ideal crypto law for liquidity pools

Uniswap is a Constant Product Market Maker built around liquidity pools, where pairs of tokens are exchanged subject to a fee that is proportional to the size of transactions. At the time of writing, there exist more than 6,000 pools associated with Uniswap v3, implying that empirical investigations on the full ecosystem can easily become computationally expensive. Thus, we propose a systematic workflow to extract and analyse a meaningful but computationally tractable sub-universe of liquidity pools. Leveraging on the 34 pools found relevant for the six-months time window January-June 2022, we then investigate the related liquidity consumption behaviour of market participants. We propose to represent each liquidity taker by a suitably constructed transaction graph, which is a fully connected network where nodes are the liquidity taker's executed transactions, and edges contain weights encoding the time elapsed between any two transactions. We extend the NLP-inspired graph2vec algorithm to the weighted undirected setting, and employ it to obtain an embedding of the set of graphs. This embedding allows us to extract seven clusters of liquidity takers, with equivalent behavioural patters and interpretable trading preferences. We conclude our work by testing for relationships between the characteristic mechanisms of each pool, i.e. liquidity provision, consumption, and price variation. We introduce a related ideal crypto law, inspired from the ideal gas law of thermodynamics, and demonstrate that pools adhering to this law are healthier trading venues in terms of sensitivity of liquidity and agents' activity. Regulators and practitioners could benefit from our model by developing related pool health monitoring tools.

==> 4-physics-previous.tex <==
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

\subsection{Model: from the ideal gas law of thermodynamics to the ideal crypto law for pools}

In Physics, an ideal gas is a theoretical gas composed of many randomly moving particles with negligible volume that are not subject to interparticle interactions. On the other hand, real gases occupy space and  molecules interact between themselves.
\dhm{We define an ideal gas as a physical system that obeys the \textit{ideal gas law}}
%Ideal gases obey the \textit{ideal gas law}, which says that
\begin{equation}
    PV = nRT, 
\label{ideal-gas-law}
\end{equation}
where $P$ is the pressure of the gas, $V$ its volume and $T$ its temperature. Furthermore, $n$ denotes the constant number of moles of particles in the considered closed system, and $R$ is the gas constant. Despite being very simple and elegant, this law describes very well \dhm{rich} dynamics.

\begin{table}[b]
\centering
\begin{tabular}[c]{ |p{1.5cm}|p{3cm}||p{3cm}|p{6cm}|  }
 \hline
 \rowcolor{LightCyan}
 \multicolumn{2}{|c||}{Ideal gas law} &\multicolumn{2}{|c|}{Ideal crypto law} \\
 \hline
 \cellcolor{Gray} Symbol & \cellcolor{LightGray} Meaning & \cellcolor{Gray} Symbol & \cellcolor{LightGray} Meaning\\
 \hline
 \hline
 $P$ & pressure & $P_{vol}$ & daily USD volume traded by LTs\\
 \hline
 $V$ & volume & $V_{stab}=\textsc{std(Z)}^{-1}$ & daily stability of the exchange rate $Z$\\
 \hline
 $n$ & moles of particles & $n_{fee} = feeTier^{-1}$ & stimulus to LTs' activation\\
 \hline
 $R$ & gas constant & $R_{pool}$ & pool crypto constant \\
 \hline
 $T$ & temperature & $T_{liq}$ & daily liquidity, i.e. proxyTVL value\\
 \hline
\end{tabular}
\vspace{0.2cm}
\caption{Parallelism drawn between the ideal gas law and our ideal crypto law.}
\label{table:ideal-crypto-law}
\end{table}


Our intuition finds resemblances between the law in Eq. \eqref{ideal-gas-law} and the crypto ecosystem, and we consider an analogy in which each pool is a gas. To define the similitude between variables that is summarised in Table \ref{table:ideal-crypto-law}, we follow how the ideal gas law was discovered and reason about both the possible meaning of variables and expected relationships.
%
First of all, $P$ can be intuitively compared to the USD volume traded by active LTs over e.g. a day.
If everything else but $T$ is kept constant, then we expect $T$ to increase with higher $P$. Therefore, we can interpret $T$ as the liquidity of the pool, i.e. the value of our proxyTVL in USD for the pool at that date. 
Indeed, the evolution of liquidity of a pool accounts for the behaviour of LPs, and more LPs should execute mint operations when there are more LTs active, in order to collect higher profit from the fees that the latter pay for each swap transaction. Clearly, we also expect a stronger overall volume traded by LTs with more liquidity, due to more convenient, smaller price impact.
%
Variable $V$ is then the volume of the gas in the thermodynamics interpretation, i.e. ideal gas law. Despite being a more subtle relationship, we find that it is reasonable to consider $V$ as the stability of the exchange rate between the two tokens in the pool, i.e. $\textsc{std(Z)}^{-1}$, where $Z$ is the exchange rate.
Keeping everything else constant, one would expect that, with higher liquidity, the price is more stable. Similarly, a compressed gas with small volume will be less stable than an expanded gas. 
In addition to that, the \textit{concentrated liquidity} mechanism of Uniswap v3 implies that LPs encounter the risk of no gains from LTs' fees if the exchange rate moves outside the range of prices over which they are actively providing liquidity. Thus, a more stable $Z$ for the same USD volume traded by LTs (i.e. $P$) is likely to attract more minting operations, especially close to the current rate.
%
Finally, a higher $P$ with the same level of liquidity is indeed likely to cause a less stable relative price of the tokens, due to the impact of surplus swap operations.

Keeping the above in mind, Eq. \eqref{ideal-gas-law} thus becomes
\begin{equation}
\begin{split}
    P_{vol} \cdot V_{stab} &= n_{fee} \cdot R_{pool} \cdot T_{liq} \\
    \Rightarrow P_{vol} \cdot \textsc{std(Z)}^{-1} 
    &= feeTier^{-1} \cdot R_{pool} \cdot T_{liq},  \\
\end{split}
\label{ideal-crypto-law}
\end{equation}
allowing us to bring together into a single formula, all the variables that govern the three mechanisms of liquidity consumption, provision, and exchange rate evolution. 
Constant $R_{pool}$ is instead the invariant characteristic of each pool, \dhm{inferred from data}. Here, $n$ is the fixed number of moles (molecules), thus   a constant. A higher $n$ means more interactions \dhm{per unit of time} in the physical description, which we relate to lower feeTier and stronger activity of the LTs, that we know dominate LPs. Thus, we express $n=feeTier^{-1}$, which is indeed constant too.

\mc{  
\paragraph{Real gases and  van der Waals forces.} 
Our above model is based on the thermodynamics law for ideal gases. However, it is worth mentioning that  there also exists  a law for real gases that interact via van der Waals forces. This is governed by the  Van der Waals equation
\begin{equation}
    \Big( P+a\frac{n^2}{V^2} \Big) \cdot (V-nb) = nRT,
\end{equation}
where the variables have same meaning as before. In addition, $a$ is a constant whose value depends on the gas and represents intermolecular forces, while $b$ is the volume occupied by the molecules of one mole of the gas.
Based on a preliminary analysis, we believe it could be of interest to  expand the ideal crypto law in this direction; however, this is beyond the scope of our current work, and we leave this for future investigation.} 

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

\subsection{Regression analysis and interpretation of results} 

As a first step, we test for empirical instances that support the validity of our ideal crypto law given by Eq. \eqref{ideal-crypto-law}.
We focus on case $A$ and consider the intersection of pools that are relevant for both liquidity provision and liquidity consumption. This results in a set of $16$ pools, namely USDC-USDT/100, WBTC-WETH/500, WETH-USDT/3000, WETH-ENS/3000, MATIC-WETH/3000, WBTC-USDC/3000, WBTC-WETH/3000, DAI-WETH/500, UNI-WETH/3000, SHIB-WETH/3000, USDC-USDT/500, USDC-WETH/500, WETH-CRV/10000, LINK-WETH/3000, USDC-WETH/3000, WETH-USDT/500.

For each individual pool, we compute the quantities $P_{vol}, V_{stab}, T_{liq}$ reported in Table \ref{table:ideal-crypto-law} at daily scale for the full six-months time window between January and June 2022. We suggest not to use higher frequencies due to significant general low rate of activity of LPs. We then scatter-plot these daily realisations for each combination of pairs of variables and critically analyse the results. Observations  with z-score $>3$ in absolute value are considered outliers and discarded. A few representative examples of the results are shown in Fig. \ref{fig:pairs-physics}, where we observe hints that the ansatz relationships are indeed satisfied, apart for the case of pools whose tokens are both stablecoins. The latter dissimilarity is perhaps not surprising, since our ideal crypto law aims at encompassing the full ensemble of crypto mechanisms, while the behaviour of LTs on pools of stablecoins has lower relevance. 
%Therefore, we proceed by focusing only on pools whose tokens are indeed not both stablecoins.


\begin{figure}[t]
\centering
\begin{subfigure}[t]{.75\textwidth}
    \centering
    \includegraphics[width=\linewidth]{physics/USDC-WETH-3000.png}
      \label{fig:sub1-crypto-law}
      \caption{USDC-WETH/3000 pool.}
\end{subfigure}    \\
\vspace{0.3cm}
\begin{subfigure}{.75\textwidth}
    \centering
    \includegraphics[width=\linewidth]{physics/UNI-WETH-3000.png}
      \label{fig:sub2-crypto-law}
      \caption{UNI-WETH/3000 pool.}
\end{subfigure}    \\
\vspace{0.3cm}
\begin{subfigure}{.75\textwidth}
    \centering
    \includegraphics[width=\linewidth]{physics/USDC-USDT-100.png}
      \label{fig:sub3-crypto-law}
      \caption{USDC-USDT/100 pool.}
\end{subfigure}    
\caption{Visualisation of pair relationships from our ideal crypto law for a sample of pools. From left to right for each case, we plot first $V_{stab}$ vs. $P_{vol}$, then $T_{liq}$ vs. $P_{vol}$, and finally $T_{liq}$ vs. $V_{stab}$.}
\label{fig:pairs-physics}
\end{figure}


We broaden our sub-universe of venues of interest by taking the union of pools significant to LTs' and LPs' behaviour in case $A$. After \dm{filtering}
%\MC{filtering or what is being checked?}
for relevance of the samples in the daily frequency, we are left with a set of $32$ pools.
%
For each pool, we perform a linear regression over the available six months of daily values, and thus estimate $R_{pool}$ by rearranging Eq. \eqref{ideal-crypto-law} to
\begin{equation}
\begin{split}
    P_{vol} &= R_{pool} \cdot \Big( \frac{ n_{fee} \cdot  T_{liq} }{V_{stab}} \Big) \\
    \Rightarrow y_{pool} 
    &= R_{pool} \cdot x_{pool},  \\
\end{split}
\label{rearrange}
\end{equation}
where the intercept is zero. We compute the coefficient of determination $R^2$ of the regression, which we refer to as the  \textit{cryptoness} $\xi$. Thus, pools with high cryptoness are meant to adhere well to our proposed ideal crypto law model.
We compute the average $\xi_{SS}$ over the seven pools found to exchange only stablecoins in our sub-universe, and compare it to the average $\xi_{notSS}$ of all other pools. We find values of $\xi_{SS} = -0.44$ and $\xi_{notSS} = -0.21$, meaning that SS pools should not be considered in our model, as expected and already motivated.
For the remaining pools, we show in Fig. \ref{fig:long-regression-a} the ones that have $\xi >0$.
We notice that different feeTiers appear to be relevant and that there is one interesting occurrence of two pools, both with high $\xi$, that exchange the same tokens, i.e. WBTC-WETH/3000 and WBTC-WETH/500. This latter result raises the question of whether these two pools are generally adhering to our ideal crypto law, or if they might follow it at disjoint periods of time that however influence the overall cryptoness values and render them both significant. Before investigating this idea further, it is worth  highlighting the fact that several pools with high $\xi$ are seen to exchange exotic tokens.
Examples are pools trading CRV and UOS, which are respectively the tokens of the well-know DEX Curve.fi, and of the blockchain-based gaming company Ultra.
The general pattern that we read is that pools exchanging digital assets linked to a tangible and established business idea might adhere better to our ideal crypto law.
%hinting at the idea that they are interpreted as equity investments. 
We think of such pools\dhm{, and companies, as being strongly embedded} in the crypto ecosystem, at least over the time window of reference in our  analyses.



For the sake of clarity, we explicitly depict in Fig. \ref{fig:long-regression-b} the linear regression pursued for the pool with highest cryptoness, i.e. WETH-CRV/10000, where occurrences that happened more recently in time are color-coded darker.
We also mention that pools might exhibit  a less good fit to our ideal crypto law due to noise introduced by the characteristic frequency of executed swaps, mint and burn operations on each pool.
Liquidity provision events are generally rare, as reported in Table \ref{table:frequencies}. Thus, it might become necessary to define ad-hoc frequencies, possibly dynamic, to be used in the regression for each pool, in order to better investigate the related evolution of behaviours.


\begin{table}[h]
\centering
\begin{tabular}[c]{ |p{3cm}|p{1.5cm}||p{3cm}|p{1.5cm}|p{3cm}|p{1.5cm}|  }
 \hline
 \rowcolor{LightCyan}
 \multicolumn{2}{|c|}{Liquidity consumption} &\multicolumn{4}{|c|}{Liquidity provision} \\
 \hline
 \cellcolor{Gray} Pool & \cellcolor{LightGray} Daily Swap & \cellcolor{Gray} Pool & \cellcolor{LightGray} Daily Mint & \cellcolor{Gray} Pool &\cellcolor{LightGray} Daily Burn\\
 \hline
 \hline
 \rowcolor{green}
 USDC-WETH/500 & 6181 & USDC-WETH/3000 & 95 & USDC-WETH/3000 & 70\\
 \hline
 \rowcolor{green}
 WETH-USDT/500 & 2395 & USDC-WETH/500 & 65 & USDC-WETH/500 & 70\\
 \hline
 \rowcolor{green}
 DAI-WETH/500 & 817 & WBTC-WETH/3000 & 19 & WBTC-WETH/3000 & 26\\
 \hline
 \hline
 \rowcolor{orange}
 WETH-CRV/10000 & 55 & DYDX-WETH/3000 & 1.0 & FXS-WETH/10000 & 1.4\\
 \hline
 \rowcolor{orange}
 USDC-UOS/10000 & 39 & USDC-UOS/10000 & 0.6 & USDC-UOS/10000 & 1.0\\
 \hline
 \rowcolor{orange}
 SHIB-WETH/10000 & 32 & CEL-WETH/3000 & 0.4 & CEL-WETH/3000 & 0.8\\
 \hline
\end{tabular}
\vspace{0.2cm}
\caption{Average daily frequency of operations on different pools for the time window of case $A$. We report the first and last three values when sorting by magnitude.}
\label{table:frequencies}
\end{table}

\begin{figure}[t]
\centering
\begin{subfigure}{.45\textwidth}
    \centering
    \raisebox{4mm}[0pt][0pt]{
    \includegraphics[width=0.8\linewidth]{physics/ranking.png}
    }
    \caption{Ranking of pools with cryptoness $\xi>0$.} 
      \label{fig:long-regression-a}
\end{subfigure}% 
\begin{subfigure}{.50\textwidth}
    \centering
    \includegraphics[width=0.75\linewidth]{physics/regression-WETH-CRV10000.png}
    \caption{The $x_{pool},y_{pool}$ values for WETH-CRV/10000 pool, which has highest $\xi$. Dots are colour-coded to encode the temporal evolution, with lighter (resp. darker) ones denoting earlier (resp. more recent) observations. The straight line denotes the linear regression line.}   
    \label{fig:long-regression-b}
\end{subfigure}    
\caption{For each pool under analysis, the linear regression between $x_{pool},y_{pool}$ is computed for daily values over the six months of case $A$. Each related coefficient of determination provides the cryptoness $\xi$ of the pool.} 
\end{figure}








\paragraph{\dhm{Dynamic} analyses.} We now analyse the evolution of our proposed  cryptoness metric for the set of pools, over the six-months time window of case $A$, i.e. Jan-June 2022. \mc{We again compute the regression in Eq. \eqref{rearrange} and record the related coefficient of determination as the cryptoness value $\xi$, but we now use the observations  contained in a $30$-day window in time, sliding every day.
This allows us to recognise pools that adhere more or less to our ideal crypto law at different points in time, and investigate the patterns generated. Interesting results for specific subsets of pools are shown in Fig. \ref{fig:physics-temporal-regressions}, where we threshold all the irrelevant $\xi < 0$ % \rightarrow
to $\xi = 0$ for ease of visualisation.
In reference to our ranking of Fig. \ref{fig:long-regression-a} and related discussion, we consider in Fig. \ref{fig:exotic-reg} the evolution of $\xi$ for a subset of pools exchanging exotic tokens, which % however
relate to well-established blockchain-based companies. As expected, we observe $\xi$s that are strongly significant for almost the entire six-months time range under consideration. Thus, we confirm that the exotic tokens depicted are deemed by our model to have solid associated companies by the dynamics of market participants and price, and we construe the related pools as \textit{healthy} venues for trading. }

\begin{figure}[t]
\centering
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{physics/EXOTIC-reg.png}
    \caption{Evolution of $\xi$ for a sample of pools exchanging exotic tokens.}
      \label{fig:exotic-reg}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{physics/SHIB-reg.png}
    \caption{Evolution of $\xi$ for two pools exchanging SHIB-WETH.}
      \label{fig:shib-reg}
\end{subfigure}    
\vspace{0.3cm}
\begin{subfigure}{.6\textwidth}
    \centering
    \includegraphics[width=\linewidth]{physics/WETH-reg.png}
    \captionsetup{width=1.2\textwidth}
    \caption{Evolution of $\xi$ for a sample of pools exchanging WETH vs. stablecoin. The dominance of different pools over time can lead to hypothesise cryptoness as a measure of the varying health of pools and indicator of where market participants should prefer to be active on.}
      \label{fig:weth-reg}
\end{subfigure}  
\caption{Evolution of cryptoness $\xi$ for different subsets of pools, where $\xi$ is now repeatedly computed from the regression over a 30-days window of instances, sliding one day each time.}
\label{fig:physics-temporal-regressions}
\end{figure}


\dm{Our intuition then suggests that there should exist \textit{only one ideal feeTier per point in time, for the exchange of two same tokens}. This feeTier would be the key that balances the set of mechanisms we are modeling and the beliefs of the market participants. 
As a first related example, Fig. \ref{fig:shib-reg} shows some association between the drops in cryptoness of the liquidity pool SHIB-WETH/10000, and the peaks in cryptoness of SHIB-WETH/3000, allowing us to consider our cryptoness measure as an indicator of the described tendency.
With a similar view, we also expect
the redundancy of pools exchanging the same token against different stablecoins to reduce the overall health of single pools, due to the related fragmentation of market participants' dynamics. 
Thus, we believe that a natural stabilisation of each token to one specific stablecoin per period in time should also be reached with the stronger establishment of crypto ecosystems.}

\dm{The results of this section provide supporting evidence towards the above concepts. In particular, we show that our cryptoness measure signals the healthiest venues (i.e. liquidity pools) where agents should be active on, by comparing simultaneous changes in $\xi$, versus variations in agents' activity and TVL. This is performed for the set of relevant pools that exchange WETH against stablecoins, i.e. DAI-WETH, WETH-USDT and USDC-WETH, also with different feeTiers, i.e. 500 and 3000.} 
Figure \ref{fig:weth-reg} shows the related evolutions of the cryptoness measure, where we can clearly see that feeTier 3000 is the relevant one for each pair DAI-WETH, WETH-USDT and USDC-WETH for the \mc{entire time window, except during April 2022.  Interestingly, over this month, no liquidity pools exhibit  strong cryptoness, except for  DAI-WETH/500, which we thus claim to be the only healthy venue for trading at that point in time. 
To support our claim}, we compute the average daily number of swap actions, mint operations and burn operations, for each one of our six pools under analysis, as related measures of activity and good usage. 
In particular, we compute average quantities over the month of April, and then over the time window Jan-June 2022 but excluding April, and then calculate the percentage change. This results in the set of values
\begin{equation}
    opChange = \frac{opApril-opNotApril}{opNotApril},
\end{equation}
where \say{op} indicates an operation between swap, mint and burn. The actual computations are reported in Fig. \ref{fig:physics-heatmap}, where we further include \textit{avgChange} as the average of \textit{swapChange}, \textit{mintChange} and \textit{burnChange}. 
%
In addition, we also plot in Fig. \ref{fig:physics-tvl} the evolution of TVL in USD over the pools of interest, in order to be able to compare occurrences of drops in liquidity over time.
Figure \ref{fig:physics-heatmap} reveals that DAI-WETH/500 is indeed the liquidity pool with the least damage of activity during April 2022. While there exists another pool which performs better than others, namely USDC-WETH/500, it suffered from a significant drop in liquidity in April 2022. On the other hand, DAI-WETH/500 had constant TVL during this month, as clearly shown in Fig.  \ref{fig:physics-tvl}.
\mc{We conclude that the only pool with a significant cryptoness $\xi$ score during April 2022 is indeed the healthiest and preferred trading venue  during the month of relevance. This provides further empirical motivation and utility} to our proposed ideal crypto law. 

Our measure of cryptoness of liquidity pools aims at becoming a useful tool for market participants, allowing them to assess the health of trading venues and decide the best environments on which to be active. 
Ideally, we would like to witness smooth dynamics of the evolution of cryptoness in the future, with new pools adhering better to the ideal crypto law once they %\MC{they or?} 
become well-rooted components of the crypto ecosystem.
From a \mc{regulatory} point of view, % ad-hoc 
dynamic requirements could then be imposed, such as less over-collateral required for trades on pools with cryptoness above a certain threshold. 
%
\mc{This metric could thus be employed both by regulators and practitioners for developing pool health monitoring tools, and establishing minimum
levels of requirement.}  
%
Finally, we believe that it would also be interesting to investigate and interpret variations in the characteristic constant $R_{pool}$ for specific pools, after drops in cryptoness. As a motivating example, Fig. \ref{fig:evol-r-pool} shows two regressions over the first and second three months of case $A$, where clearly the slope of the recovered lines varies significantly.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[h]
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[width=.99\linewidth]{physics/change-weth-stablecoin-heatmap.png}
      \caption{Variation in activity, i.e. in the frequency of the different transaction types, over April.} 
      \label{fig:physics-heatmap}
    \end{subfigure}%
    \begin{subfigure}{.6\textwidth}
      \centering
      \includegraphics[width=.99\linewidth]{physics/tvl-weth-stablecoin.png}
      \caption{Our proxyTVL in USD.}
      \label{fig:physics-tvl}
    \end{subfigure}
    \caption{Comparison of activity variation and liquidity evolution between our six pools exchanging WETH against a stablecoin, over the six months of case $A$. We discuss changes in average activity over April 2022 versus on the remaining five months of case $A$, and similarly compare disequilibria of minting versus burning operations in USD traded.     Pool DAI-WETH/500 is the only venue of the subset with significant cryptoness in April 2022 and indeed, it reports both the least damage in activity and no drop in proxyTVL over that month.}
    \label{fig:physics-final}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{physics/shib-r-evolve.png}
    \caption{A pool that shows the evolution in time of its characteristic coefficient $R_{pool}$. The yellow and green lines are generated from the regressions over data from the first three months, or last three months respectively, for case study $A$.} 
    \label{fig:evol-r-pool}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%


